Analysis and Detection of Information Types of Open Source Software Issue Discussions

Most modern Issue Tracking Systems (ITSs) for open source software (OSS) projects allow users to add comments to issues. Over time, these comments accumulate into discussion threads embedded with rich information about the software project, which can potentially satisfy the diverse needs of OSS stakeholders. However, discovering and retrieving relevant information from the discussion threads is a challenging task, especially when the discussions are lengthy and the number of issues in ITSs are vast. In this paper, we address this challenge by identifying the information types presented in OSS issue discussions. Through qualitative content analysis of 15 complex issue threads across three projects hosted on GitHub, we uncovered 16 information types and created a labeled corpus containing 4656 sentences. Our investigation of supervised, automated classification techniques indicated that, when prior knowledge about the issue is available, Random Forest can effectively detect most sentence types using conversational features such as the sentence length and its position. When classifying sentences from new issues, Logistic Regression can yield satisfactory performance using textual features for certain information types, while falling short on others. Our work represents a nontrivial first step towards tools and techniques for identifying and obtaining the rich information recorded in the ITSs to support various software engineering activities and to satisfy the diverse needs of OSS stakeholders.

==> discussion.tex <==
% \section{Discussion}



==> future_work.tex <==
\section{Future Work}
The work done in this paper is the first step towards an automated technical comment and sentence information identification system. The interesting results that identification can be done with an F1 of 61\% motivates future work in this domain. To begin with, we plan to research the effect of using word embeddings on general and domain-specific data to vectorize text and retrieve more metdata-based contextual features for representing the data. Additionally deep learning models for text classification such as neural networks have proven to perform better than previous state-of-the-art methods\cite{Lai:2015:RCN:2886521.2886636}, and hence are worth exploring. Ultimately, we hope to summarize sentences belonging to similar information types in an issue thread to allow potential users to obtain quickly the gist of the discussion with respect to their information requirement.


%We plan to explore deeply Topic modeling  Future work includes improvement in topic modeling (on larger dataset maybe), clustering, increased feature set, Leave-One(Document)-Out Cross Validation using word2vec or word embeddings and different oversampling techniques like GLOVE, trying different algorithms like LSTM and deep models for classification. Further, summarization of the sentences in the different classes to produce coherent summaries for different purposes and potential viewers and readers of the issue thread discussion.


==> topic_modeling.tex <==
\section{Unsupervised Information Type Detection}
As the manual effort involved in the comment labeling process is non-trivial, we pursue the possibility of identify information types through unsupervised method, i.e. topic modeling.

Topic modeling is the process of identifying "topics" or themes present in a collection of documents. The algorithm creates clusters of similar words based on the frequency statistics of each word. Additionally, a document generally comprises of multiple topics, hence, topic modeling indicates the proportion of multiple topics present in a document based on the proportion of words present in each topic in the document. For example, a document containing the words 'bug' and 'problem' will likely be about a bug report whereas the words 'solution and 'fixed' will occur more often in a document about a solution to a problem. If a document is 80\% about a reported bug and 20\% about the way to fix it, the ratio of words about the bug to those about the fix will also be 80:20. This is the premise of topic modeling.

Latent Dirichlet Allocation (LDA) is a graphical-based topic modeling algorithm in which every document is believed to have a small set of topics each identified by a small set of terms which occur frequently\cite{Blei2003}. The topics in LDA are modelled on this assumption of document contents and the produced topic distribution based on this assumption is known as a Dirichlet prior.

\subsection{Data Filtering and Preprocessing}
Since topic modeling is an unsupervised mechanism, the lack of necessity of labelled data allowed us to perform LDA on all closed issues in the three projects, tensorflow, scikit-learn and spaCy, combined. For our experiments, each comment was treated as a singe "document". Hence our dataset comprised of a total of \hilight{XX} comments from \hilight{XX} issues. The preprocessing performed on these comments were the same as in supervised learning, described in Section \ref{data_preprocessing}.

\subsection{Feature Set Preparation}
To perform topic modeling, it is necessary to vectorize the comments. As in the supervised classification, each comment was tokenied into words using the spaCy English word tokenizer, followed by lemmatization, lowercasing and removal of punctuation and common contractions. The set of words in a comment were then transformed into numerical representation using their term frequencies as required by the LDA algorithm.

\subsection{Experimental Design}
%In order to measure the topic modeling capabilities on the dataset, we attempted to perform LDA on a total of X comments obtained from Y issues from the 3 projects - tensorflow, scikit-learn and spaCy.

We performed LDA topic modeling on the extensive dataset. The LDA algorithm requires an input of the number of topics ($k$) to be identified in the input. Evaluation of unsupervised learning for topic count has been of much discussion, especially for the purpose of determining the best hyperparameter in an experimental setting. The general methods are usually comparison with a golden truth set\cite{Wallach:2009:EMT:1553374.1553515} or human evaluation\cite{W15-1526}. However our lack of a labelled extensive dataset and the inconvenience of human evaluation on different hyperparamater runs limits our ability to use these techniques.
In our work, we use a stability metric to assess the performance of the topic modeling algorithm over different number of topics. This is done using a term-based approach to calculate the similarity between the top $n$ terms in topics for different subsets or samples of the dataset. The higher the similarity value for the topics, the better is the hyperparameter used. This model was introduced by Green et al. in their work\cite{Greene2014}. We use their tool\footnote{https://github.com/derekgreene/topic-stability} to experiment with stability of top 3-15 terms for topic counts between 4 and 12.

\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{images/topic_modeling_stability.pdf}
    \caption{Stability of topic modeling via LDA for different k values. }
    \label{fig:topic_stability}
\end{figure}

\subsection{Results and Discussion}
Figure \ref{fig:topic_stability} shows the stability for the top $n$ terms per $k$ topics. Though all stability values are low, it is observed that $k=6$ performs the best on average for the top 3 to 15 terms.
